Strategic investments in multi-stage General Lotto games

In adversarial interactions, one is often required to make strategic decisions over multiple periods of time, wherein decisions made earlier impact a player's competitive standing as well as how choices are made in later stages. In this paper, we study such scenarios in the context of General Lotto games, which models the competitive allocation of resources over multiple battlefields between two players. We propose a two-stage formulation where one of the players has reserved resources that can be strategically pre-allocated across the battlefields in the first stage. The pre-allocation then becomes binding and is revealed to the other player. In the second stage, the players engage by simultaneously allocating their real-time resources against each other. The main contribution in this paper provides complete characterizations of equilibrium payoffs in the two-stage game, revealing the interplay between performance and the amount of resources expended in each stage of the game. We find that real-time resources are at least twice as effective as pre-allocated resources. We then determine the player's optimal investment when there are linear costs associated with purchasing each type of resource before play begins, and there is a limited monetary budget.

==> backup/model.tex <==
Consider a two-stage game with players $A$ and $B$, who compete over a set of $n$ battlefields, $\mcal{B}$. Each battlefield $b\in\mcal{B}$ is associated with a valuation $w_b > 0$, which is common to both players. Player $A$ is endowed with a monetary budget $X_A > 0$ for which to purchase two types of resources in the first stage -- \emph{stationary} and \emph{mobile} resources. The per-unit cost for investing in stationary resources is $c \geq 0$, and the per-unit cost for investing in mobile resources is $c_m = 1$. Player $B$ is endowed with $M_B > 0$ mobile resources, which it can only employ in the second stage.

In the first stage, player $A$ decides how many stationary and mobile resources to purchase. In particular, it selects a pair $(S,M_A)$ that satisfies
\begin{equation}\label{eq:monetary}
    cS + M_A \leq X_A, \quad (S,M_A) \in \mbb{R}_+^2.
\end{equation}
At the end of the first stage, player $A$ decides how to allocate the $S$ stationary resources to the battlefields: it selects a vector $\bs{s} = (s_1,\ldots,s_n) \in \Delta_n(S) := \{\bs{s}' \in \mbb{R}_+^n : \|\bs{s}'\|_1 = S \}$. The vector $\bs{s}$ is referred to player $A$'s \emph{pre-allocation}. Player $B$ makes no decisions in this stage, as we assume that it does not have access to stationary resources. No payoffs are derived in stage 1.

In stage 2, players $A$ and $B$ compete in a simultaneous-move General Lotto game over $\mcal{B}$ with their mobile budgets $M_A,M_B$. Here, both players can randomly allocate these resources as long as their expenditure does not exceed their budgets in expectation. Specifically, a strategy for player $\ell \in \{A,B\}$ is an $n$-variate (cumulative) distribution $F_\ell$ over allocations $\bs{x}_\ell \in \mbb{R}_+^n$ that satisfies
\begin{equation}\label{eq:LC}
    \mbb{E}_{\bs{x}_\ell \sim F_\ell}\left[\sum_{b\in\mcal{B}} x_{\ell,b} \right] \leq M_\ell.
\end{equation}
We denote $\mcal{L}(M_\ell)$ as all strategies $F_\ell$ that satisfy \eqref{eq:LC}. Given that player $A$ has the pre-allocation $\bs{s}$ from stage 1, the expected payoff to player $A$ is given by
\begin{equation}
    u_A(F_A,F_B) := \mbb{E}_{\substack{\bs{x}_A \sim F_A \\ \bs{x}_B \sim F_B}}\left[ \sum_{b\in\mcal{B}} w_b \cdot I(x_{A,b}, qx_{B,b}- s_b) \right]
\end{equation}
where\footnote{The tie-breaking rule can be assumed to be arbitrary, without affecting any of our results. This property is common in the General Lotto games literature \cite{Kovenock_2020,Vu_EC2021}} $I(a,b) := 1(a > b)$ for any two numbers $a,b \in \mbb{R}_+$. In other words, player $B$ must overcome player $A$'s pre-allocated resources $s_b$ as well as player $A$'s allocation of mobile resources $x_{A,b}$ in order to win battlefield $b$. The parameter $q > 0$ is the quality of player $B$'s mobile resources against player $A$'s. When $q < 1$ ($q > 1$), they are less (more) effective than player $A$'s resources. The payoff to player $B$ is $u_B = nw - u_A$.

We will denote an instance of the second-stage sub-game as $\text{LF}(\bs{s},M_A,M_B)$, which is a General Lotto game with favoritism \cite{Vu_EC2021}. An equilibrium of $\text{LF}(\bs{s},M_A,M_B)$ is a profile $(F_A^*,F_B^*) \in \mcal{L}(M_A)\times\mcal{L}(M_B)$ that satisfies
\begin{equation}
    \begin{aligned}
        u_A(F_A^*,F_B^*) &\geq u_A(F_A,F_B^*) \text{ and} \\ 
        u_B(F_A^*,F_B^*) &\geq u_B(F_A^*,F_B)
    \end{aligned}
\end{equation}
for any $F_A \in \mcal{L}(M_A)$ and $F_B\in\mcal{L}(M_B)$. The recent literature has shown that an equilibrium exists in any instance of this game \cite{Vu_EC2021}, and the equilibrium payoff is unique. There, they formulated numerical methods to calculate an equilibrium with arbitrary precision. We will denote the unique equilibrium payoffs to the players as $\pi_A(\bs{s},M_A,M_B)$ and $\pi_B(\bs{s},M_A,M_B)$.

\subsection{Optimal investment problem}

We are interested in characterizing player $A$'s optimal investment decision $(S^*,M_A^*)$ as well as the optimal pre-allocation $\bs{s}^*$ in stage 1, such that its equilibrium payoff in the stage 2 sub-game is maximized. Specifically, we seek to solve the optimization problem
\begin{equation}\label{eq:investment_problem}
    \pi_A^* := \max_{(S,M_A) : cS+M_A \leq X_A} \max_{\bs{s} \in \Delta_n(S)} \pi_A(\bs{s},M_A,M_B)
\end{equation}
where recall that $c \geq 0$ is the per-unit cost to invest in stationary resources, $X_A$ is the total monetary budget of player $A$, and $M_B>0$ is the amount of player $B$'s mobile resources.

{\color{red} We are interested in the best pair $(S^*,M_A^*)$ subject to some resource allocation constraint, and denote the payoff to player $A$ as $\pi^*_A$.

Examples of scenarios... linear cost model... norms (e.g., max-norm)... cone constraint... robust optimization (incomplete information)...}

%%

In the \emph{General Lotto game with favoritism} (GL-F) \cite{Vu_EC2021}, two players $A$ and $B$ with respective budgets $X_A, X_B\geq 0$ compete over a set of $n$ battlefields $\mcal{B}=\{1,\dots,n\}$.  Every battlefield $b\in\mcal{B}$ has an associated value $w_b>0$ that is common to both players, and an offset $f_b\in\mbb{R}$.  An admissible strategy for each player $i\in\{A,B\}$ is any $n$-variate distribution $\mcal{F}_i$ on $\mbb{R}^n_+$ that satisfies 
\begin{equation} \label{eq:lotto_budget_constraint}
    \mbb{E}_{\mathbf{x}_i \sim \mcal{F}_i} \left[ \sum_{b\in\mcal{B}} x_{i,b} \right] \leq X_i.
\end{equation}

\noindent In words, each player $i\in\{A,B\}$ can select any distribution $\mcal{F}_i$ over allocations $\mathbf{x}_i = (x_{i,1}, \dots, x_{i,n})^T \in\mbb{R}^n_+$ as long as it satisfies her budget in expectation.  For given allocations $\mathbf{x}_A, \mathbf{x}_B\in\mbb{R}^n_+$, we say that player $A$ wins battlefield $b\in\mcal{B}$ if $x_{A,b}+f_b>x_{B,b}$, and that player $B$ wins $b$ otherwise.\footnote{The tie-breaking rule (i.e., deciding who wins if $x_{A,b}+f_b=x_{B,b}$) can be assumed to be arbitrary, without affecting any of our results. This property is common in the General Lotto games literature, see, e.g., \cite{Kovenock_2020,Vu_EC2021}.}  Each player's payoff is the expected sum over the values of battlefields that she wins.  Observe that an instance of GL-F can be succinctly represented as a tuple $\{X_A,X_B,\mathbf{w},\mathbf{f}\}$, where we let $\mathbf{w}\in\mbb{R}^n_{++}$ and $\mathbf{f}\in\mbb{R}^n$ denote the vectors of battlefield values and offsets, respectively.

We note that the terminology of favoritism stems from the offset parameter $f_b\in\mbb{R}$ on each battlefield $b\in\mcal{B}$.  Indeed, if $f_b>0$, then  battlefield $b$ ``favors'' player $A$ as player $A$ can win $b$ even in situations where $x_{A,b}<x_{B,b}$.  Similarly, if $f_b<0$, then $b$ favors player $B$.  As one might expect, the classic General Lotto game model (without favoritism) is equivalent to the GL-F game where $f_b=0$ for all $b\in\mcal{B}$.

For a given GL-F instance $G=\{X_A,X_B,\mathbf{w},\mathbf{f}\}$, let $\pi_i(\mcal{F}_A, \mcal{F}_B; G)$, $i\in\{A,B\}$, denote the players' payoffs for admissible player strategies $\mcal{F}_A$, $\mcal{F}_B$.  Then, an equilibrium of $G$ is a pair of admissible strategies $\mcal{F}^*_A$, $\mcal{F}^*_B$ that satisfies
\begin{equation}
\begin{aligned}
    \pi_A(\mcal{F}^*_A, \mcal{F}^*_B; G) &\geq \pi_A(\mcal{F}_A, \mcal{F}^*_B; G), \; \forall \text{ admissible } \mcal{F}_A, \\
    \pi_B(\mcal{F}^*_A, \mcal{F}^*_B; G) &\geq \pi_B(\mcal{F}^*_A, \mcal{F}_B; G), \; \forall \text{ admissible } \mcal{F}_B.
\end{aligned}
\end{equation}

\noindent For any given GL-F game $G$, it has recently been shown that an equilibrium exists, and that the equilibrium payoffs $\pi^*_i(G) = \pi_i(\mcal{F}^*_A, \mcal{F}^*_B; G)$, $i\in\{A,B\}$, are unique \cite{Vu_EC2021}.  The same authors also formulate numerical methods to calculate an equilibrium and the corresponding payoffs. 

%%

\subsection{Optimal investment problem}

% The initial study of the GL-F game model was entirely devoted to proving existence of equilibrium and providing an equilibrium characterization.  
In this manuscript, we seek to extend the analysis to settings where favoritism is the result of strategic investment by one of the players prior to the competitive interaction.  To that end, we define the following two-stage variation on the GL-F game, where we assume that players' choices made in a given stage are binding, and become common knowledge in subsequent stages:

\smallskip\noindent--\emph{Stage 1:} Player $A$ selects a pair $(S,M_A)\in\mcal{I}(X_A)\subseteq\mbb{R}^2_+$, and, subsequently, a vector $\mathbf{s}\in\Delta_n(S)$;

\smallskip\noindent--\emph{Stage 2:} Players $A$ and $B$ play $\text{GL-F}(M_A,X_B,\mathbf{w},\mathbf{s})$, and receive the corresponding payoffs.

\smallskip\noindent These two stages are illustrated in \Cref{fig:main_figure}a.  Intuitively, in Stage 1, player $A$ chooses how to invest her budget in \emph{stationary} ($S$) and \emph{mobile} ($M_A$) resources while respecting a budget constraint $(S,M_A)\in\mcal{I}(X_A)$ to be specified.  After selecting her investment, player $A$ allocates her acquired stationary resources among the battlefields in $\mcal{B}$.  Then, in Stage 2, the players play a GL-F game in which the offsets stem from $A$'s allocation of her stationary resources in Stage 1.  We assume that both players' choices are made to maximize their respective payoffs in Stage 2.

Note that we do not endow player $B$ with the ability to invest in stationary resources, and, thus, all of her budget $X_B$ enters as mobile resources.  To make this clear, we will use $M_B=X_B$ to denote player $B$'s budget throughout.

We are interested in characterizing player $A$'s optimal Stage 1 choices, i.e., the investment $(S^*, M_A^*)\in\mcal{I}(X_A)$ and subsequent allocation $\mathbf{s}^*\in\Delta_n(S^*)$ that maximize her equilibrium payoff in the ensuing GL-F game played in Stage 2.  Formally, given $X_A, M_B\geq0$ and $\mathbf{w}\in\mbb{R}^n_{++}$, we wish to solve the following optimization problem:  
\begin{equation} \label{eq:optimal_investment_problem}
    \underset{(S,M_A)\in\mcal{I}(X_A)}{\text{maximize}} \enspace 
    \underset{\mathbf{s}\in\Delta_n(S)}{\text{maximize}} \enspace
    \pi^*_A(M_A,M_B,\mathbf{w},\mathbf{s}).
\end{equation}

\noindent Clearly, the optimal choice $(S^*, M_A^*)$ depends on the budget constraint $\mcal{I}(X_A) \subseteq \mbb{R}^2_+$. However, we have not yet specified an expression for the set $\mcal{I}(X_A)$.  This is because there are many problems with distinct budget constraints that fall under this structure.  We provide a few examples of optimal investment problems, as well as expressions for their corresponding sets $\mcal{I}(X_A)$, below:

\begin{example}[Linear cost constraint] \label{ex:linear_cost}
    Consider the setting where player $A$'s choice in Stage 1 must satisfy a linear cost constraint, i.e., 
    \begin{equation} \label{eq:linear_cost_constraint}
        \mcal{I}(X_A) = \{(S,M_A)\in\mbb{R}^2_+ \text{ s.t. } M_A + cS \leq X_A\},
    \end{equation}

    \noindent where $c\geq 0$ represents the relative cost of stationary resources to mobile resources.  
\end{example}

\begin{example}[Relative effectiveness of pre-allocated resources] \label{ex:relative_effectiveness}
    Consider the setting where player $A$'s choice in Stage 1 must satisfy a constraint of the form $\mcal{I}(X_A) = \{(X_A/c,0), (0,X_A)\}$, where $c\geq 0$ represents the relative cost of pre-allocated to real-time resources.  By analyzing this constraint, we study the relative effectiveness of pre-allocated and mobile resources when deployed in isolation.
\end{example}

In the above examples, observe that $c<1$ corresponds with settings where stationary resources are ``cheaper'' than mobile resources.  Thus, for $c \geq 1$ (i.e., when stationary resources are more expensive), we immediately expect the optimal choice to be $(S^*,M^*_A) = (0,X_A)$.
% The standard approach for solving such two-stage games is to identify the Stage 1 choices that maximize the analytical expression for player $A$'s payoff in Stage 2.  Since Stage 2 consists of a GL-F game, the players' payoffs resulting from player $A$'s choices in Stage 1 are unique, and a sub-game perfect equilibrium can be computed using the numerical methods provided in \cite{Vu_EC2021}.  However, to derive player $A$'s optimal investment in Stage 1, we require an \emph{analytical} expression for player $A$'s equilibrium payoff in Stage 2, which is missing from the literature.  This gap, along with other analytical challenges associated with the optimization problem in \eqref{eq:optimal_investment_problem}, prompts the following questions that we seek to address in this paper:

% {\color{red} Trick: We bypass the requirement for an exact analytical characterization of players' equilibrium payoffs in Stage 2 by solving for the optimal $\bs{s}^*$ directly.}


==> backup/results.tex <==
% % % % PROOF of optimal investment in linear cost model. DONT DELETE
% \begin{proof}
%     We first observe that for any $\Pi \in (0,W)$, the level curve $R_A^\Pi(P)$ (from Theorem \ref{thm:level_set}) is strictly decreasing and convex in $P \in [0,\frac{qR_BW}{W-\Pi}]$, where we use $R_A^\Pi(P)$ to explicitly note the dependence on $\Pi$. Hence, the function $\pi_A(P,R_A,R_B)$ is quasi-concave in $(P,R_A)$.  Observe that the set of points $(P,R_A)\in\mbb{R}^2_+$ that satisfy $R_A + cP = X_A$ consists of the line segment $R_A=X_A-cP$, $P\in[0,X_A/c]$, with slope $-c$, and end-points $(X_A,0)$ and $(0,X_A/c)$.  Thus, the optimization amounts to finding the highest level curve that intersects with $R_A=X_A-cP$, $P\in[0,X_A/c]$.  
    
%     The slope of a level curve $R_A^\Pi(P)$ at $P=0$ is
%     \begin{equation}
%         \frac{\partial R_A^\Pi}{\partial P}(0) =
%         \begin{cases}
%             -\frac{2\Pi}{W}, &\text{if } \Pi < \frac{W}{2} \\
%             -1, &\text{if } \Pi \geq \frac{W}{2}
%         \end{cases}.
%     \end{equation}
%     Let $X_A\geq0$ such that $\pi^*_A(0,X_A,R_B)=\Pi\geq W/2$.  Then, note that, if $-c<-1$ (or, equivalently $c>1$), then $R_A=X_A-cP$ shrinks faster in $P$ than the level curve $R_A^\Pi(P)$ by monotonicity and convexity of the level curve in $P$.  Thus, the allocation $(P,R_A)=(0,X_A)$ maximizes $A$'s payoff, as all other points on the line segment $R_A=X_A-cP$, $P\in[0,X_A/c]$, intersect with strictly lower level curves.  Similarly, for $X_A\geq0$ such that $\pi^*_A(0,X_A,R_B)=\Pi<W/2$, the allocation $(P,R_A)=(0,X_A)$ maximizes $A$'s payoff when $c>2\Pi/W$.  Since the condition $\pi^*_A(0,X_A,R_B)=\Pi\geq W/2$ is equivalent to $X_A\geq qR_B$ and $\pi^*_A(0,X_A,R_B)=WR_A/(2 qR_B)$ when $X_A<qR_B$, it follows that $P^*=0$ if $c>\min\{1,X_A/(qR_B)\}$.  For the remainder of the proof, we use $t=1$ (resp. $t=X_A/(qR_B)$) and $X_A\geq qR_B$ (resp. $X_A<qR_B$) interchangeably.
%     % Suppose $c > t$ and $t = \frac{X_A}{qR_B}$ (resp. $t=1$). The level curve corresponding to $\pi^*_A(P,X_A-cP,R_B) = \frac{WX_A}{2qR_B}$ (resp. $\pi^*_A(P,X_A-cP,R_B) = W(1 - \frac{qR_B}{2X_A})$) has a single budget-feasible point at $P=0$. For any level curve corresponding to $\Pi > \Pi(X_A)$, there are no budget-feasible points. Hence, $P^*=0$.
    
%     Suppose that $c = t$ and $t = \frac{X_A}{qR_B}$. Then the level curve corresponding to $\Pi(X_A) = \frac{W}{2}c$ has an interval of budget-feasible points $(P,R_A)$ parameterized by $P \in [0,(1-\frac{c}{2-c})\frac{X_A}{c}]$ with $R_A = X_A - cP$. If $t = 1$, then there is a single budget-feasible point $(P,R_A) = (0,X_A)$ for the level curve corresponding to $\Pi(X_A) = W(1-\frac{qR_B}{2X_A})$. In both cases, there are no budget-feasible points for any level curve corresponding to $\Pi > \Pi(X_A)$. 
    
%     Now, suppose $c < t$ and $t = 1$. We wish to find the level curve for which the line $(P,X_A-cP)$, $P \in [0,X_A/c]$, lies tangent. The point(s) of tangency yields the optimal solution due to the quasi-concavity of $\pi_A^*$. Furthermore, since $X_A\geq qR_B$ and $c < 1$, a solution $(P,R_A)$ must satisfy $\Pi \in [\frac{W}{2},W]$ and
%     \begin{equation}\label{eq:tangent_point}
%         \begin{aligned}
%             \frac{\partial R_A^\Pi}{\partial P}(P^*) &= \frac{P^*(W-\Pi)}{qR_BW} - 1 &&= -c \\
%             R_A^\Pi(P^*) &= \frac{(qR_BW - (W-\Pi)P^*)^2}{2qR_BW(W-\Pi)} &&= X_A - cP^*
%         \end{aligned}
%     \end{equation}
    
%     \noindent From the first equation, we obtain $P^* = \frac{qR_BW(1-c)}{W-\Pi}$. Plugging this expression into the second equation, we obtain $\Pi = W(1 - \frac{qR_B}{2X_A}c(2-c)) \in [\frac{W}{2},W]$, which leads to the unique solution $P^* = (1-\frac{c}{2-c})\frac{X_A}{c} \leq \frac{X_A}{c}$.
    
%     Lastly, suppose $c < t$ and $t = \frac{X_A}{qR_B}$ ($X_A < qR_B$). Similar to the preceding case, we seek the highest level curve for which the budget constraint is tangent. Due to the assumption that $X_A < qR_B$ and $c < \frac{X_A}{qR_B}$, we observe that tangent points cannot exist for $P < \frac{W-2\Pi}{W-\Pi}qR_B$ and $\Pi < \frac{W}{2}$, i.e. in the region where the level curve is linear. Thus, it must be that either $\Pi < \frac{W}{2}$ and $P \geq \frac{W-2\Pi}{W-\Pi}qR_B$, or $\Pi \geq \frac{W}{2}$. In either case, a solution must also satisfy the equations in \eqref{eq:tangent_point}, from which we obtain an identical expression for $P^*$.
% \end{proof}
% % % % END proof of linear cost investment % % % % % %
    

% With abuse of notation, we will denote the payoff to player $A$ when $P$ is optimally allocated in Stage 2 as $\pi^*_A(R_A,R_B,\bs{w},P)$, i.e., for given $P, R_A, R_B>0$, let
% \[ \pi^*_A(R_A,R_B,\bs{w},P) := \pi_A(R_A,R_B,\bs{w},\bs{p}^*). \]

% \noindent Thus, the optimization problem in \eqref{eq:optimal_investment_problem} reduces to
% \begin{equation}\label{eq:reduced_investment_problem}
%     \pi_A^\mathrm{opt} = \max_{(P,R_A)\in\mcal{I}(X_A)} \pi^*_A(R_A,R_B,\bs{w},P).
% \end{equation}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEVEL CURVES PROOF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
We leverage the expression for player $A$'s equilibrium payoff from \Cref{thm:equilibrium_characterization}.  First, observe that, for $R_A=0$ and $P\geq qR_B$, player $A$'s payoff is
\[ \pi^*_A(P,0,R_B) = W \cdot \left( 1-\frac{qR_B}{P} \right), \]
from which we extract the fact that $\pi^*_A(P,R_A,R_B)>\Pi$ for all $R_A\geq0$ when $P>WqR_B/(W-\Pi)$.

We continue by noting that if $qR_B\geq P$ and $R_A<\frac{2(qR_B-P)^2}{P+2(qR_B-P)}$, then $\pi^*_A(P,R_A,R_B)=W\cdot R_A/(2(qR_B-P))$, and it immediately follows that
\[ R_A = \frac{2\Pi}{W} (qR_B-P). \]

\noindent From this expression for $R_A$, the condition $R_A<\frac{2(qR_B-P)^2}{P+2(qR_B-P)}$ can be reduced to
\[\begin{aligned}
    && \frac{2\Pi}{W} (qR_B-P)     &< \frac{2(qR_B-P)^2}{P+2(qR_B-P)} \\
    % \frac{2\Pi}{W} (2qR_B-P)    &< 2(qR_B-P) \\
    % [2 - 2\Pi/W] P              &< [2 - 4\Pi/W] qR_B \\
    % (W-\Pi) P                   &< (W-2\Pi)qR_B \\ 
    \iff \> && P                           &< \frac{W-2\Pi}{W-\Pi} qR_B.
\end{aligned}\]

\noindent The right-hand side of the last line must be less than or equal to $qR_B$, and, thus, satisfies $qR_B\geq P$.  The condition $P\geq0$ provides the lower bound in \eqref{eq:level_curve_1and2}, and, when $W<2\Pi$, it precludes $P<\frac{W-2\Pi}{W-\Pi}qR_B$.  Thus, $R_A=\frac{2\Pi}{W}(qR_B-P)$ when $\Pi<W/2$ and $P\in[0,\frac{W-2\Pi}{W-\Pi}qR_B)$.

Next, we consider the case where either $qR_B<P$, or $qR_B\geq P$ and $R_A\geq\frac{2(qR_B-P)^2}{P+2(qR_B-P)}$.  In this case, $A$'s payoff $\pi^*_A(P,R_A,R_B)=\Pi$ is given by \eqref{eq:allcase1_payoff}. This expression can be simplified as follows:

% \[ W\cdot\left(1 - \frac{qR_B}{2R_A}\left(\frac{R_A + \sqrt{R_A(R_A+2P)}}{P+R_A+\sqrt{R_A(R_A+2P)}} \right)^2 \right). \]

\[\begin{aligned}
         && \Pi &= W \frac{P+f-qR_B}{P+f} \\
    % \iff && \Pi (P+f) &= W (P+f-qR_B) \\
    \iff && f &= \frac{(W-\Pi)P-W qR_B}{\Pi-W}
\end{aligned}\]

\noindent where we denote $f := R_A+\sqrt{(R_A+P)^2-P^2}$.  By substituting the expression for $f$ into the last line, rearranging and squaring both sides, we get:
\[\begin{aligned}
    (R_A+P)^2-P^2   &= \left( g - R_A \right)^2, % \\
    % (R_A)^2 + 2R_AP &= g^2 - 2 g R_A + (R_A)^2
\end{aligned}\]

\noindent from which we obtain $R_A = g^2/(2(P+g))$, where we denote $g := \frac{(W-\Pi)P-W qR_B}{\Pi-W}$.  Substituting for $g$ and simplifying gives the expression
\begin{equation} \label{eq:ma_case1}
    R_A = \frac{(qR_BW-(W-\Pi)P)^2}{2qR_B(W-\Pi)W}.
\end{equation}

\noindent This is the expression for $R_A$ either when $qR_B\geq P$ and $R_A\geq\frac{2(qR_B-P)^2}{P+2(qR_B-P)}$, or $qR_B < P$.  From the former, we get the condition:
\[ \frac{((qR_B-P)W+\Pi P)^2}{2qR_B(W-\Pi)W} 
    \geq \frac{2(qR_B-P)^2}{2qR_B-P}, \]

\noindent which simplifies to the expression $P\geq qR_B\frac{W-2\Pi}{W-\Pi}$.  Finally, if $qR_B<P$, then the expression for $R_A$ in \eqref{eq:ma_case1} holds for all $P\in[0,qR_B\frac{W}{W-\Pi}]$.
\end{proof}
